A Quantitative Evaluation Framework for Missing Value Imputation Algorithms

We consider the problem of quantitatively evaluating missing value imputation algorithms. Given a dataset with missing values and a choice of several imputation algorithms to fill them in, there is currently no principled way to rank the algorithms using a quantitative metric. We develop a framework based on treating imputation evaluation as a problem of comparing two distributions and show how it can be used to compute quantitative metrics. We present an efficient procedure for applying this framework to practical datasets, demonstrate several metrics derived from the existing literature on comparing distributions, and propose a new metric called Neighborhood-based Dissimilarity Score which is fast to compute and provides similar results. Results are shown on several datasets, metrics, and imputations algorithms.

==> ApproachOLD.tex <==

%In many real world machine learning and data mining applications, data often contain missing values. While ignoring examples with missing elements is one option, 
%this results in throwing away some valuable information such examples could provide. This paper concerns learning to impute missing values given a partially filled 
%data matrix. There have been several approaches presented in the literature. Include some references starting from EM approach for handling incomplete data, Zoubin's work, conditional and joint modeling approaches (our known existing literature survey on missing values including non-probabilistic models), some literature on matrix factorization, matrix filling, etc. (our related work section (say, section 2) should cover all these topics).

\section{Evaluation Approach}
In this section, we provide details of the three key parts given in algorithm ${\mathcal A}$: (1) Model construction and sample generation (steps A and B1) (section 3.1), (2) Score computation using metrics (step B3) (section 3.2) and (3) Ranking of algorithms with statistical significance testing (step B4 and C) (section 3.3). We make the following assumptions: (a) there are at least a reasonable number of examples with no missing values; this is true in many practical scenarios, (b) a conditional probabilistic model powerful enough to capture the underlying distribution can be built using these examples, and (c) generating samples from the model distribution can be done easily via Gibbs sampling. \\ 
\noindent{\bf Notations} Let ${\mathcal D}_N$ and ${\mathcal D}_M$ denote the sets of examples with no missing values and with missing values respectively. Let ${m}_j \subset \{1,\cdots,d\}$, $j=1,\cdots,J$ denote a subset of variables for which values are missing in ${\mathcal D}_M$ with $d$ denoting the number of variables. Note that each subset $m_j$ refers to a unique missing pattern and there are $J$ missing patterns in ${\mathcal D}_M$. Also, let $o_j = \{1,\cdots,d\} \setminus m_j$. Let $Y^{(i)}_{m}$ and $Y^{(i)}_{o}$ denote the missing and observed variables in the $i^{th}$ example respectively. 
 
\subsection{Distribution Model Learning}
The first step is to build a distribution model such that for each missing pattern $m_j$, we can generate samples given the values for the corresponding observed pattern $o_j$. We can build a joint model $P(Y;\theta)$ using the set ${\mathcal D}_N$ (where $\theta$ is the model parameter). However, building such a joint model is hard and intractable; more importantly, it is not necessary. This is because we always have some observed variables that can be used to predict the missing variables. Furthermore, conditional models are relatively easier to build. Due to these reasons, we build conditional distribution model $P(Y_{m_j}|Y_{o_j};\theta_j)$ for each missing pattern $m_j$ in ${\mathcal D}_M, \forall j$ using the fully observed data set ${\mathcal D}_N$; $\theta_j$ denotes the $j^{th}$ model parameter vector. \\
\noindent{\bf Model and Learning} While any decent conditional model is sufficient for our method to work, we use pairwise Markov random field (MRF) for illustrative purpose. For ease of notation, we will remove the subscript in $m_j$. We use the model: 
%\begin{equation}
%\vspace{0.1in}
$P(Y_m|Y_o;\theta) = \frac{1}{Z(Y_o)} \exp(s(Y_m;\theta_m) + s(Y_{m};Y_{o},\theta_{mo}))$
%\label{condmodel}
%\end{equation}
where $Z(Y_o) = \sum_{Y_m} \exp(s(Y_m;\theta_m) + s(Y_{m};Y_{o},\theta_{mo}))$ is the partition function and, $s(Y_m;\theta_m)$ and $s(Y_{m};Y_{o},\theta_{mo})$ denote parametrized scoring functions involving self and cross features among the missing and observed variables. In our experiments, we use a simple linear model for the scoring function: $s(Y_m;\theta_m) = \sum_{k \in m} \sum_{{\bar y}_{k,l} \in {\mathcal Y}_k} \theta_{k,l} {\mathcal I}(y_{k} = {\bar y}_{k,l})$ where ${\mathcal Y}_k$ is the label space for the $k^{th}$ variable and ${\mathcal I}(\cdot)$ is the indicator feature function. The scoring function $s(Y_{m};Y_{o},\theta_{mo})$ is defined using similar feature functions involving a pair of variables and associated parameters. Given a missing pattern $m$, we construct a training set comprising of input-target pairs $\{(Y^{(i)}_o,Y^{(i)}_m):i=1,...,n\}$ from ${\mathcal D}_N$ and learn the model parameter $\theta$ using the piecewise pseudo-likelihood maximization training approach suggested by Sutton and McCallum (2008).

%is learned by solving the following optimization problem: 
%\begin{equation}
%\argmax_{\theta} {\mathcal H}(\theta) = -\lambda \frac{||\theta||^2}{2} + \frac{1}{n} \sum_{i=1}^n \log P(\bfymi|\bfyoi;\theta)
%\label{optfncond}
%\end{equation}
%where $\lambda$ is a regularization parameter. Note that $\log P(\bfymi|\bfyoi) =  \symi + \symoi - \log Z(\bfyoi)$. The difficulty in solving this problem arises due to computational intractability of $Z(\bfyoi)$ (when $\bfym$ is high dimensionality and/or the number of state combinations is too many) and its gradient. We overcome this difficulty by using the piecewise pseudo-likelihood maximization training approach suggested by Sutton and McCallum (2008). 
\noindent{\bf Multiple Imputations} Using the model parameters learned for each missing pattern $m_j$, we generate multiple imputations for each example in ${\mathcal D}_M$ (having the missing pattern $m_j$) via Gibbs sampling. For instance, sample generation for a discrete variable involves sampling a multinomial distribution with probabilities that can be easily computed from the conditional MRF distribution. 

\noindent{\bf Single Model} One disadvantage of the above modeling is that we need to build $J$ conditional models. However, these models can be built in parallel and is one time effort. On the other hand, we can build a single conditional model that can be used for any missing pattern. The key difference is that we learn a single model parameter vector $\theta$ (instead of learning one model parameter vector $\theta_j$ per missing pattern $m_j$). In this case, there is only one dataset and log likelihood term for each example involves different missing pattern. Therefore, the subset of linear model parameter $\theta$ described above could be different depending on the variables involved, and parameter overlapping happens across the examples. Building a single model helps in reducing the computational complexity. Though such a model is expected to be inferior in prediction quality compared to per missing pattern model, we found this to be adequate to meet the requirement of ranking the methods correctly.

\subsection{Metrics}
Given samples $(Y_m)$ from the model (\textit{true}) conditional distribution $(P)$ and multiple imputations $({\hat Y}_m)$ obtained from an imputation algorithm $k$ (with its distribution ${\hat P}_{k}$), we compute a score for samples $(Y_m,{\hat Y}_m)$ from each pair $(P,{\hat P}_k)$. In this section we describe several popular metrics (selected from the literature) that we use to compute the score and compare in our experiments. These metrics measure the discrepancy between samples generated from $(P,{\hat P})$. (For ease of notation, we drop the dependency on algorithm $k$ in ${\hat P}_k$ in the discussion below).  

\noindent{ \bf KL divergence via Convex Optimization} Estimation of divergence functionals and likelihood ratios using samples generated from two probability distributions $(P, \hat P)$ is an important problem in machine learning and information theory. Nguyen et al (2010) shows that this estimation problem can be posed as an empirical risk minimization problem and solved using standard convex programs. Computing KL divergence is an instantiation of this problem and we use their approach to compute the KL divergence between the multiple imputation samples obtained for each missing pattern. In particular, we solve the following optimization problem: 
\begin{equation}
- min_{\alpha > 0} F = - \frac{1}{L} \sum_{u=1}^L log(L \alpha_u) + \frac{1}{2\lambda_L L} g(\alpha,Y_m,{\hat Y}_m)
\label{eq:KLD}
\end{equation}
where $\lambda_L$ is a regularization constant, $L$ is the number of imputation samples, $g(\alpha,Y_m,{\hat Y}_m) = \sum_{u,v} \alpha_u \alpha_v K(y^{(u)}_m,y^{(v)}_m) + \frac{1}{L} K({\hat y}^{(u)}_m,{\hat y}^{(v)}_m) - \sum_{u,v} \alpha_v \alpha_j K(y^{(u)}_m,{\hat y}^{(v)}_m)$ and $K(\cdot, \cdot)$ is a kernel function. We used the Gaussian kernel $K(y,{\hat y}) = \exp(-||y-{\hat y}||^2/\sigma)$ and set the kernel width parameter $\sigma$ to $1$ in our experiments. Finally, the KL divergence value is computed using the solution ${\hat \alpha}$ obtained from solving (\ref{eq:KLD}) as: $-\frac{1}{L}\sum_{u=1}^L log(L {\hat \alpha}_u)$.

\noindent{\bf Symmetric KL divergence via binary classification} It is known that the KL divergence is not symmetric with respect to the distributions used, and, it is often useful to consider Jensen-Shannon divergence having the symmetric property (defined as: $\frac{1}{2}(KL(P,\frac{P+{\hat P}}{2}+KL(P,\frac{P+{\hat P}}{2})$). While it is theoretically possible to adapt the estimation approach suggested by Nguyen et al (2012) to estimate the symmetric KL divergence, it does not result in a simpler convex program like (\ref{eq:KLD}). It is interesting to note that Reid et al (2011) developed a unified framework to show that many machine learning problems can be viewed as binary experiments and estimation of various divergence measures can be done by solving a binary classification problem with suitably weighted loss functions for the two categories. In our context, we found that the symmetric KL divergence can be estimated as follows: (a) assign class labels +1 and -1 for the samples from the model distribution and imputation algorithm respectively, and, (b) build a classifier using standard logistic loss function. The intuition is that more divergent the distributions easier the classification task. Therefore, the error rate measures the discrepancy between the distributions.   
 
\noindent{\bf Maximum Mean Discrepancy} Gretton et al (2012) proposed a framework in which a statistical test can be conducted to compare samples from two distributions. The main idea is to compute a statistic known as maximum mean discrepancy (MMD) and use an asymptotic distribution of this statistic to conduct a hypothesis test ${\mathcal H}_0: P = {\hat P}$ with a suitably defined threshold. The MMD statistic is defined as supremum over the mean difference between some function score computed from the samples of respective distributions. They show that functions from reproducing kernel Hilbert space (RKHS) are rich to compute this statistic from finite samples and derive conditions under which MMD can be used to distinguish the distributions. Given the MMD function class ${\mathcal F}$ the unit ball in a RKHS ${\mathcal H}$ with kernel $K(y,{\hat y})$ (e.g., Gaussian), the statistic is defined as: 
\begin{equation}
{\hat MMD}^2_u({\mathcal F},Y_m,{\hat Y}_m) = g_{yy}(Y_m) + g_{{\hat y}{\hat y}}({\hat Y}_m) - g_{y{\hat y}}(Y_m,{\hat Y}_m)
\label{eq:mmd}
\end{equation}
where $$g_{y{\hat y}}(Y_m,{\hat Y}_m) = \frac{1}{L(L-1)} \sum_{u=1}^L\sum_{v\ne u}^L K({y}^{(u)}_m,{\hat y}^{(v)}_m);$$ $g_{yy}(Y_m)$ and $g_{{\hat y}{\hat y}}({\hat Y}_m)$ are similarly defined. To reduce the computational complexity and produce low variance estimates in the finite sample issue associated with computing (\ref{eq:mmd}), Zaremba et al (2013) propose a statistical test known as B-test. With this theoretical backing, we include two metrics: (a) the statistic MMD and (b) the B-test result to rank the algorithms in our study. The B-test gives $0$ or $1$ as the output (with $1$ indicating acceptance of ${\mathcal H}_0$); therefore, there will be ties. However, the rank aggregation algorithm that we describe in section~\ref{sec:RA} can handle this. 

%propose a family of tests called B-tests where an average statistic is computed as follows: (a) divide $L$ samples into $\frac{L}{B}$ blocks of size $B$, (b) compute the statistic $\eta_l$ using (\ref{eq:mmd}) for $l^{th}$ block and (c) average the computed statistics as: $\eta = \frac{B}{L} \sum_{l=1}^\frac{L}{B} \eta_l$. Using the result $\eta \rightarrow {\mathcal N}(MMD^2,\sigma^2_u)$ where $MMD^2$ is defined in expectation sense ($(\ref{eq:mmd})$ is an empirical estimate) with $(P, {\hat P})$ and variance $\sigma^2_u$ computed using the eigen value equations involving kernels. Choice of kernel parameters play an important role in minimizing type II error for a given type I error in the hypothesis testing. See Gretton et al (2012) and Zaremba et al (2013) for more details. With this theoretical backing, we include two metrics: (a) the statistic $(\eta)$ and (b) the B-test result to rank the algorithms in our study. Note that the B-test gives $0$ or $1$ as the output (with $1$ indicating acceptance of ${\mathcal H}_0$); therefore, there will be ties. However, the rank aggregation algorithm that we describe in section~\ref{sec:RA} can handle this. 
 
\noindent{\bf Neighborhood Dissimilarity Score} One disadvantage of the above metrics is that they are computationally expensive since we need to solve the associated problems for each example in ${\mathcal D}_M$. This becomes an issue when $J$ is large. We propose a neighborhood dissimilarity score (NDS) that is cheaper to compute and is defined as: 
\begin{equation}
nds(h,Y_m,{\hat Y}_m) = \frac{1}{L^2}\sum_{u=1}^L \sum_{v=1}^L w_{uv} h(y^{(u)}_m,{\hat y}^{(v)}_m)
\label{eq:nds}
\end{equation}
where $h(\cdot)$ is a distance score (e.g., Hamming loss) computed between a pair of examples on the imputed values and $w_{uv}$ is a weighting factor given by: $\lambda^{h(\cdot)} + (1-\lambda)^{(h_{max} - h(\cdot))}$; $\lambda$ and $h_{max}$ denote a scaling parameter and maximum Hamming distance possible. Note that $w_{uv}$ gives more weight to neighbors and $\lambda$ controls the rate at which the weight falls off in terms of distance. We used $\lambda=0.1$ in our experiments.  Though it is quadratic in $L$, $L$ is typically small (e.g., 25) and the overall complexity is $O(JL^2)$. NDS is closely related to (\ref{eq:mmd}) with three key differences: (a) we consider only the cross terms, (b) there are no kernel parameters to learn in NDS, and (c) the weighting is not uniform ($w_{uv}$ compared to uniform weighting of $\frac{1}{L(L-1)}$ used in (\ref{eq:mmd})). Our experimental results show that NDS is a good metric in the sense of producing results similar to MMD and KL based metrics.     
\subsection{Rank Aggregation}
Given a metric ${\mathcal M}$ and algorithm $k \in {\mathcal A}$ (a set of algorithms to compare), we compute the score $s^{(i)}_{k,{\mathcal M}}$ for $i^{th}$ example in ${\mathcal D}_M$ using procedures presented in the previous section. Using the scores, we rank the algorithms for each $i$ resulting in a rank matrix ${\mathcal R}_{\mathcal M}$ with each column representing the ranks of an algorithm in ${\mathcal A}$. To compare the algorithms, we draw analogy to the problem of statistically comparing multiple classifiers over multiple datasets (Demsar, 2006). In particular, we treat multiple imputations for each example as one dataset and we have scores for $|{\mathcal D}_M|$ datasets for a given algorithm and metric. Our goal is to statistically compare the performance of algorithms in ${\mathcal A}$ on these datasets. Following Demsar (2006), we conduct Friedman test with the null hypothesis that all algorithms are equivalent. This test involves computing the average ranks of each algorithm, and computing a statistic and checking against ${\mathcal X}^2_F$ distribution for a given confidence level $\beta$ (we used 0.05). It turned out that the null hypothesis is always rejected for the algorithms that we considered. So, we conducted Nemenyi test as the post-hoc test (Demsar, 2006). In this test, we compute critical difference (CD) score defined as: $q_{\beta} \sqrt{\frac{|{\mathcal A}|}{|{\mathcal D}_M|}}$ where $q_{\beta}$ is obtained from a look-up table. The observed average rank difference between any two methods is statistically significant when it is greater than CD. We demonstrate this in our experiments later and make key observations. 

\label{sec:RA}
%\noindent{\bf Assumptions}
%\begin{enumerate}
%\item Ground truth data is available.
%\item Imputation method under evaluation generates multiple imputations and/or gives probability distribution of the missing values for each example (record) (say, 
%$\pmi$). 
%\item When the probability distribution is known, we can generate the samples (keeping the observed values fixed) using Gibbs sampling.
%\end{enumerate}
%\subsection{Proposed Approach}
%The proposed approach consists of two steps:
%\begin{enumerate}
%\item find the probability distribution of the missing values for each example (having missing values) (say, $\qmi$) using the ground truth data, and 
%\item compute a quality metric that computes difference between $\pmi$ and $\qmi$ (e.g., KL-divergence or Jensen-Shannon divergence) for each example and aggregates over the examples. (In this step, instead of comparing $\pmi$ and $\qmi$, we could use samples generated from these distributions and compute other metrics such as maximum mean discrepancy (MMD) score described in Gretton {\it et al}, (2012) paper.) 
%\end{enumerate}
%
%\noindent{\bf Questions} (1) Is MMD applicable for multivariate mixed type (binary, category, ordinal, continuous) data? (2) How do we define kernel (say, Gaussian RBF or Laplace) for the mixed type data?
%
%\noindent{\bf Discussion} When the ground truth data is available, why do we need to find $\qmi$? In probabilistic modeling framework, there is no certainty in having only a single assignment of missing values given observed values of an example. In contrast, the ground truth data gives {\it one instance} or {\it one possible assignment} when several other assignments are possible. Multiple imputations generated by any imputation method attempt to bring out this uncertainty. Therefore, modeling this uncertainty through $\qmi$ using all the ground truth data {\it for each example} is important. Although the quality of the uncertainty model depends on the model space, the best information one could attempt to get is $\qmi$ conditional on the model space (since the model is built using {\it known missing values} available in the ground truth data). Therefore, using $\qmi$ as the reference model for comparison of imputation methods is a viable approach.   
%
%\noindent{\bf Remarks} As mentioned above, we still need to define a metric to compare the quality of imputations (\emph{i.e}., step 2 is still needed). This is where the metrics (e.g., Bipartite matching, Yet Another Metric, etc) that we defined earlier come into picture. For example, when we use samples from $\qmi$ and multiple imputations, these metrics can be used to compare the methods.  
%
%\subsection{Finding $\qmi$}
%One way to find $\qmi$ for each example is to use the entire ground truth data. The basic idea is to find the missing variables in the $i^{th}$ row and build a classifier model $q_i(\bfym|\bfyo)$ using all the examples, treating $\bfyoi$ and $\bfymi$ as the input and target variables respectively. There are several challenges: 
%\begin{enumerate}
%\item the number of classifier models that need to be built is equal to the number of unique combination of missing variables; although these classifiers can be built in parallel, this number can be prohibitively large.
%\item the number of state combinations in $\bfymi$ can be high; this could happen when the number of missing variables is large (e.g., high dimensional data and/or percentage of missing is high) and/or the number of states for each variable is large. In such cases, learning a probabilistic model and computing probabilities will be intractable due to the partition function. Also, learning a reliable model is not easy when there are only a few examples available.
%\item there may be several irrelevant variables in each problem and using them to learn the model can be harmful.  
%\end{enumerate}
%
%\subsubsection{Nearest Neighbor Classifier} 
%
%A simple classifier model one could use is \emph{k-nearest neighbor} classifier. Here, $k$ nearest (neighbors) examples (${\mathcal N}^{(i)}$) is found from the ground truth data using only the observed values of the $i^{th}$ example. Then, $\qmi$ can be computed as the empirical distribution of \emph{known} missing values of the examples in ${\mathcal N}^{(i)}$, \emph{i.e}., 
%\begin{equation}
%\qmi = \frac{1}{k} \sum_{j=1}^k v_j \sum_{\bfym} \delta(\bfym = \bfymj).
%\label{nnest}
%\end{equation}
%where $v_j = 1, \forall j = 1, \ldots, k$. Instead of giving equal weight to all the neighbors, one could assign different weights to each example depending on the distance between the examples in the observed part. For example, a \emph{normalized} weight that can be used is: 
%\begin{equation}
%v_j = \frac{\exp(-h(\bfyoi,\bfyoj))}{G_i}
%\label{weight}
%\end{equation} 
%where $h(\cdot)$ is the Hamming distance between the examples and $G_i = \sum_{j=1}^{k}\exp(-h(\bfyoi,\bfyoj))$. (While computing metric such as MMD, ${\mathcal N}^{(i)}$ is directly used along with the multiple imputations generated by the imputation method.) When we consider $|{\mathcal N}^{(i)}| = k = n$, we use all the examples in the ground truth data. Note that $\qmi$ is estimated using examples with different observed outputs (but, suitably weighted by the distance.) 
%
%\subsubsection{Structured Output Predictor}
%There are two other classifier models that consider. They are based on defining a Markov Random Field structure on $\bfym$ conditional on $\bfyo$. In the first model, we build one structured output predictor per example; this is computationally expensive. In the second model, we build only one structured output predictor that is applicable across all the examples. This model is cheaper to compute. However, the prediction quality may not be as good as the first model. The actual performance needs to be evaluated. Nevertheless, since the goal is to relatively rank the imputation methods, it is sufficient to build a model that is better than the imputations methods that we evaluate. We will present the details of building these predictors later after introducing necessary notations needed for MRF, piecewise training and inference in Section 3.  
%
%\subsection{Quality Metric Computation}
%\subsubsection{Using Probability Distributions}
%When the distributions $\qmi$ and $\pmi$ are available and the number of state combinations of $\bfymi$ is tractable, we could compute the symmetric KL-divergence: $\texttt{KL}(\qmi||\pmi)$. However, this poses a problem when $\pmi = 0$ for the states $\bfymi$ such that $\qmi \ne 0$. (This situation should not arise for exponential models except for numerical inaccuracy. In practice this can happen when the probability distributions are estimated using generated samples (e.g., imputed samples)). We consider the following alternatives: 
%\begin{enumerate}
%\item Compute Jensen-Shannon divergence measure: \\ $\texttt{JS}(\qmi||\pmi) = \frac{1}{2} \texttt{KL}(\qmi||r_i) + \frac{1}{2} \texttt{KL}(r_i||\pmi)$ where $r_i = \frac{1}{2}(\qmi+\pmi)$.
%\item Let us define three regions:
%\begin{enumerate} 
%\item the set of states ($D$) for which both $\qmi$ and $\pmi$ are not zero, 
%\item the set of states ($M$) for which $\qmi \ne 0$ and $\pmi = 0$, and 
%\item the set of states ($F$) for which $\qmi = 0$ and $\pmi \ne 0$. 
%\end{enumerate}
%Let $({\tilde p}_d,{\tilde q}_d)$, ${\tilde q}_m$ and ${\tilde p}_f$ denote the corresponding probabilities. Large values of ${\tilde q}_m$ and ${\tilde p}$ also indicate that the quality of imputation is not good. One simple measure is to compute weighted L2-norm using these probabilities; {\it i.e}.,
%\begin{equation}
%{\mathcal M}(\qmi,\pmi) = w_m {\tilde q}^2_m + w_f {\tilde p}^2_f + w_d ({\tilde p}_d-{\tilde q}_d)^2
%\label{sqloss}
%\end{equation} 
%where $w_m$, $w_f$ and $w_d$ are some weights that the user may be interested in assigning. (When the weights are set to 1, this is equivalent to treating each region as a class and computing MMD for the unit vector feature mapping of three classes, namely, $[0\:\:0\:\:1]$, $[0\:\:1\:\:0]$, $[0\:\:0\:\:1]$, and usual inner product.) It is also useful to compute KL divergence only in the region $D$ ({\it i.e}.,$\texttt{KL}_D(\qmi||\pmi)$) with the normalized probabilities $\frac{\pmi}{{\tilde p}_d}$ and $\frac{\qmi}{{\tilde q}_d}$ to get valid distributions. However, it is unclear how to combine the quantities ${\tilde q}_m$, ${\tilde p}_f$, (${\tilde q}_d$, ${\tilde p_d}$) and $\texttt{KL}_D(\qmi||\pmi)$ in a meaningful way to define a single measure that can be used to compare different imputation methods. 
%\end{enumerate}
%%\subsubsection{Using Samples}
%%Consider the scenarios where $\qmi$ and/or $\pmi$ are not computable due to intractability of their respective partition functions, or not available. For example, many imputation methods output only the imputed samples. Even though closed form solutions may be available for $\qmi$ and $\pmi$, we could generate samples using Gibbs sampler and use them after burn-in time. Then there are several possibilities: 
%%\begin{enumerate}
%%\item When only samples are available we could estimate the probability distribution and use measures discussed in the previous section.
%%\item Use metric such as MMD using a Gaussian RBF kernel where the kernel size $\sigma$ can be chosen as suggested in Gretton {\it et al} (2012) paper. 
%%\item Use other metrics that we considered earlier, namely, bipartite matching and Yet Another Metric. (We have not done any experiments so far).  
%%\end{enumerate}
%%We define the last two metrics below.
%%\subsubsection*{Yet Another Metric}
%%Let us refer the samples generated or obtained from the reference classifier model and imputation method as $\mcsi$ and $\mchatsi$ respectively. Then, we define the following measure for $i^{th}$ example: 
%%\begin{equation}
%%C_i = \sum_{j \in \mcsi} \frac{v_j}{|\mchatsi|} \sum_{l \in \mchatsi} {\mathcal M}({\bf y}^{(j)}_m, {\hat {\bf y}}^{(l)}_m)
%%\label{yam}
%%\end{equation}
%%where ${\mathcal M}(\cdot)$ is some measure (e.g., Hamming distance) that measures the distance between the \emph{known} or sampled missing values (${\bf y}^{(j)}_m$) obtained from $\qmi$ and imputed values (${\hat {\bf y}}^{(l)}_m$), and $v_j$ is the weight associated with the $j^{th}$ sample in $\mcsi$ ($\sum_j v_j = 1$). Finally, the overall measure is computed as an average over all the examples (\emph{i.e}., $\frac{1}{n} \sum_{i=1}^n C_i$).  
%%
%%%\noindent{\bf Bipartite Matching Metric (BMM)}
%%\subsubsection*{Bipartite Matching Metric (BMM)}
%%Using the above notations, BMM is defined as: 
%%\begin{equation}
%%B_i = \argmin_R \sum_{j \in \mcsi} \sum_{l \in \mchatsi} r_{j,l} {\mathcal M}({\bf y}^{(j)}_m, {\hat {\bf y}}^{(l)}_m)
%%\label{yam}
%%\end{equation}
%%where $R=\{r_{j,l}\}$, $r_{j,l} > 0$, $\sum_{j \in \mcsi} r_{j,l} = \frac{1}{|\mchatsi|}$ and $\sum_{l \in \mchatsi} r_{j,l} = \frac{1}{|\mcsi|}$. The overall measure is computed as an average over all the examples (\emph{i.e}., $\frac{1}{n} \sum_{i=1}^n B_i$).
%%
%%\section{Markov Random Fields, Piecewise Training and Inference}
%%Let $\bfy$ denote $K$-dimensional random (label) vector with $j^{th}$ random variable $y_j \in {\mathcal Y}_j$, where ${\mathcal Y}_j$ is the label space. Let $\bfyi$ denote the $i^{th}$ example where $i \in \{1,\ldots,n\}$. Let $\bfymi$ and $\bfyoi$ denote the missing and observed parts of $\bfyi$. We define a scoring function for a label vector $\bfy$ as:
%%\begin{equation}
%%\s = \sum_{c \in {\mathcal C}} \sc
%%\label{scfn}
%%\end{equation}
%%where $c$ and ${\mathcal C}$ denote $c^{th}$ component in a collection of components ${\mathcal C}$ in the network ${\mathcal G}$ connecting the variables in $\bfy$; $\bfyc$ and $\theta_c$ denote the $c^{th}$ component variables and associated model parameters. (In supervised learning (structured prediction) problems, we additionally have input variables $\bfx$ and the scoring function is dependent on both $\bfx$ and $\bfy$. Later, we will consider the split of missing and observed variables parts, and associated scoring function.)  
%%
%%\noindent{\bf Pairwise MRF Example} Consider a network ${\mathcal G}$ where all the variables are connected to each other, with the scoring function $\s$ defined as: 
%%\begin{equation}
%%\s = \sum_{j=1}^K \sj + \sum_{j=1}^K \sum_{k = j+1}^K \sjk
%%\label{scmrfn}
%%\end{equation}
%%where $\sj$ and $\sjk$ denote $j^{th}$ node and $(j,k)$ edge scores respectively. In linear form, they are given by: $\sj = \sum_{{\bar y}_j \in {\mathcal Y}_j} \theyj \Iyj$ where $\Iyj$ is an indicator function, and $\sjk = \sum_{{\bar y}_j \in {\mathcal Y}_j} \sum_{{\bar y}_k \in {\mathcal Y}_k} \theyjyk \Iyjk$.
%%
%%Using the scoring function, the probabilistic model is defined as: 
%%\begin{equation}
%%p(\bfy) = \frac{1}{Z} \exp(\s)
%%\label{probmodel}
%%\end{equation}
%%where $Z$ is the partition function given by $\sum_{\bfy} \exp(\s)$ and we have omitted the model parameter $\theta$ to simplify the notation. Given a set of examples $\{\bfyi:i=1,...,n\}$, the model parameter $\theta$ is learned by solving the following optimization problem: 
%%\begin{equation}
%%\argmax_{\theta} {\mathcal H}(\theta) = -\lambda \frac{||\theta||^2}{2} + \frac{1}{n} \sum_{i=1}^n \log p(\bfyi)
%%\label{optfn}
%%\end{equation}
%%where $\lambda$ is a regularization parameter. Note that $\log p(\bfyi) = \si - \log Z$. The difficulty in solving this problem arises due to computational intractable nature of the partition function $Z$ and its gradient. Sutton and McCallum suggests to solve this problem via piecewise training approach. In this approach using the decomposable nature of the scoring function (\ref{scfn}), the objective function ${\mathcal H}(\theta)$ is modified as: 
%%\begin{equation}
%%\argmax_{\theta} {\tilde {\mathcal H}(\theta)} = -\lambda \frac{||\theta||^2}{2} + \frac{1}{n} \sum_{i=1}^n \sum_{c \in {\mathcal C}} \sci - \log Z_c
%%\label{optfn1}
%%\end{equation}
%%where $Z_c = \sum_{\bfyc} exp(\sc)$ and is independent of example ({\it i.e}., there is no dependency on $i$; however, $Z_c$ is dependent on $\bfxi$ in structured prediction problems, {\it i.e}., $Z_c(\bfxi)$.). Solving this problem is computationally tractable as long as each component $c$ is tractable. Note that the only difference between (\ref{optfn}) and (\ref{optfn1}) is the partition functions involved. 
%%
%%\noindent{\bf Inference} Once the model parameters are learned, the inference problem is nothing but a discrete variables optimization problem: 
%%\begin{equation}
%%\bfy^{*} = \argmax_{\bfy} \s
%%\label{infpbm}
%%\end{equation}
%%This problem is solved using dual decomposition method (Komadakis and Paragios, CVPR, 2009; Komadakis, Paragios and Tziritas, 2007(?)).
  %%
%%\noindent{\bf Piecewise Training of pairwise MRF} For the scoring function (\ref{scmrfn}), we could define $K$ components with $j^{th}$ component score: 
%%\begin{equation}
%%\sbj = \sj + \sum_{k \ne j} \frac{\sjk}{2}
%%\label{score}
%%\end{equation}   
%%where $\bfyMj = \bfy - y_j$ ({\it i.e.,} leaving out the $j^{th}$ variable and $\s = \sum_{j=1}^K \sbj$. Note that with $\bfyMj$ fixed, $\sbj$ is only a function of single variable $y_j$. Therefore, defining the partition function $Z_j = \sum_{y_j \in {\mathcal Y}_j} exp(\sbj)$ (which is tractable), we have:  
%%\begin{equation}
%%\argmax_{\theta} {\tilde {\mathcal H}(\theta)} = -\lambda \frac{||\theta||^2}{2} + \frac{1}{n} \sum_{i=1}^n \sum_{j = 1}^K \sbij - \log Z_j. 
%%\label{optfn2}
%%\end{equation}
%%We make three observations: (1) this decomposition can be viewed as splitting the graph as a collection of $K$ trees (components) with $j^{th}$ tree (component) taking $y_j$ as the root node and $\bfyMj$ as its children, (2) the model parameters are shared across the trees as some of the edges are shared across the trees, and (3) the partition function $Z_j$ of tree is tractable since the summation is only over $y_j \in {\mathcal Y}_j$. 
%%
%%\section{Structured Output Predictor Models}
%%\subsection{Predictor Model per Missing Pattern}
%%In this case, we identify the index set ${\mathcal J}^{(i)}$ for the $i^{th}$ example. Then, treat the columns indexed by ${\mathcal J}^{(i)}$ as the targets, and use the other columns ${\bar J}^{(i)}$ as the inputs. We build one predictor model for each \emph{unique} index set. To simplify notations, let us use $\bfym$ and $\bfyo$ as the target and input variables (but, these variables change for each example depending on the index set) respectively for any example. As earlier, we build an MRF model, but a conditional model, i.e., $q(\bfym|\bfyo;\theta)$. (For simplicity, we have omitted the dependence on the index set.). We split the scoring function (\ref{scmrfn}) in terms of $\bfym$ and $\bfyo$ as: 
%%\begin{equation}
%%%\s = \sum_{y_j \in \bfym} \sj + \sum_{y_j \in \bfyo} \sj + \sum_{j=1}^K \sum_{k = j+1}^K \sjk
%%\s = \sym + \symo + \syo
%%\label{condscrfn}
%%\end{equation}
%%Note that only the first two terms contain the target variables $\bfym$ with the associated model parameters. 
%%First, note that the marginal probability $p(\bfyo;\theta)$ is given by: 
%%$$q(\bfyo;\theta) = \frac{1}{Z} \sum_{\bfym} \exp(\sym + \symo) \exp(\syo)$$ where $Z = \sum_{\bfy} \exp(\s)$. Using these expressions, the relation $q(\bfym|\bfyo) = \frac{q(\bfy)}{q(\bfyo)}$ and (\ref{probmodel}), we get: 
%%\begin{equation}
%%q(\bfym|\bfyo) = \frac{1}{Z(\bfyo)} \exp(\sym + \symo)
%%\label{condmodel}
%%\end{equation}
%%where $Z(\bfyo) = \sum_{\bfym} \exp(\sym + \symo)$. Given a set of examples $\{(\bfyoi,\bfymi:i=1,...,n\}$ (for a given index set), the model parameter $\theta$ is learned by solving the following optimization problem: 
%%\begin{equation}
%%\argmax_{\theta} {\mathcal H}(\theta) = -\lambda \frac{||\theta||^2}{2} + \frac{1}{n} \sum_{i=1}^n \log q(\bfymi|\bfyoi)
%%\label{optfncond}
%%\end{equation}
%%where $\lambda$ is a regularization parameter. Note that $\log q(\bfymi|\bfyoi) =  \symi + \symoi - \log Z(\bfyoi)$. The difficulty in solving this problem arises due to computational intractable nature of the partition function $Z(\bfyoi)$ (when $\bfym$ is high dimensionality and/or the number of state combinations is too many) and its gradient. We use the piecewise training approach discussed earlier to address this problem. 
%%
%%In (\ref{optfncond}), the index set used is same across all the examples; note that the index set is defined per missing pattern and we use all examples in the ground truth data to build a predictor model for each pattern. Therefore, the optimized model parameter values are different for each missing pattern. 
%%
%%\subsection{A Single Predictor Model}
%%The only difference between the previous model and the single predictor model is that the index set changes for each example $i$ in (\ref{optfncond}); as a consequence, the parameters involved also varies across the missing patterns. However, there is only a single model globally. 
%%


==> Conclusions.tex <==
\section{Conclusion}
We presented a framework to quantitatively evaluate and rank the goodness of imputation algorithms. It allows users to (a) work with any decent conditional modeling choice, (b) use metrics that are efficient and consistent (any improved quality metrics that appear in future as this field matures can be easily incorporated), (c) compare metrics using any new consistency checks, and (d) rank algorithms using well-laid out statistical significance tests. 
%We demonstrated the usefulness of framework with quantitative evaluation on several realworld datasets supported by motivating visual evaluation using several metrics and algorithms. 
%As a future work, it is important to evaluate on many real world datasets with different characteristics, and recommend quality imputation algorithms and metrics for different applications.

==> IntroductionOLD.tex <==
\section{Introduction}
\label{sec:intro}

% Where is multiple imputation explained/defined?

Many commonly used machine learning algorithms assume that the input data matrix does not have any of its entries missing. But in practice this is often not true. \emph{Imputation} is one popular approach to handling missing values -- it fills in the dataset by inferring them from the observed values. Once filled, the dataset can then be passed on to an ML algorithm as if it were fully observed. \emph{Multiple imputation} takes into account the uncertainty in the missing values by sampling each missing variable to produce multiple filled-in versions of the dataset. Multiple imputation has been an active area of research in Statistics and ML [refs] and has been implemented in many popular Statistics/ML packages [refs].

Although there has been much work on mulitple imputation, quantitatively measuring the relative performance of a set of imputation algorithms on a given dataset remains an open problem. In the special case where it is known ahead of time that the dataset is to be used only for a specific task (e.g. classification), one can use the evaluation metric for that task (e.g. 0/1 loss) to indirectly measure the performance of an imputation algorithm. But here we are interested in directly evaluating the quality of the imputation, without using a subsequent task for a proxy evaluation.  

%For example, if the task is classification, one can evaluate a set of imputation algorithms by using them to fill in the dataset, train a classifier on each filled-in dataset, measure the 0/1 loss achieved with each dataset, and rank algorithms accordingly\footnote{In such a case, the end task's objective function can be directly optimized even when inferring the missing values also.}. 

Current procedures available for evaluating imputations are qualitative. Some imputation tools, such as the R packages \emph{mi} and \emph{MICE}, allow visual comparison of the histogram of observed values and imputed values for each column of the dataset. Such comparisons can be done only for one or two variables at a time and so is at best a weak sanity check. van Buuren and Groothuis-Oudshoorn mention criteria for checking whether the imputations are plausible, e.g. \emph{imputations should be values that could have been obtained had they not been missing}, \emph{imputations should be close to the data}, and they should \emph{reflect the appropriate amount of uncertainty about their `true' values}. But such criteria have not yet been translated into quantitative metrics.

%, and in the worst case the missingness mechanism can be such that these two histograms are not supposed to be the same (e.g due to covariate shifts between rows with a variable missing and rows with that variable observed)

One possibility for quantifying imputation performance is to hold out a subset of observed values from the dataset, impute them, and measure the ``reconstruction error'' between the known and predicted values using an appropriate distance metric, e.g. Euclidean distance for real-valued variables and Hamming distance for categorical variables. As Rubin explains in [ref], this is not a good metric because there can be uncertainty in the value of the missing variables (conditioned on the values of the observed variables), and directly comparing imputed samples to a single groundtruth value cannot measure this uncertainty. 

%As a simple example, suppose that a set of rows differ only by the value of a single held out variable that can take on two equally probable values. Any imputation that assigns the two values equally often to the held out variable (which in effect correspond to different permutations of the rows) are equally valid, but reconstruction error will not be the same for them. 

The key quantity needed to evaluate an imputation is the \emph{distribution of the missing variables conditioned on the observed variables}.  Consider a data vector $Y$ with observed variables $Y_{obs}$ and missing variables $Y_{mis}$, with $Y = \{Y_{obs},Y_{mis}\}$. Let $R$ be a vector of indicator variables indicating which variables in $Y$ are missing or not. As explained in Little and Rubin (Chapter 11, page 219, equation 11.4), the joint distribution of $Y$ and $R$ can be written as
\begin{align*}
P(Y,R) &= P(Y|R)P(R)\\
&= P(Y_{mis},Y_{obs}|R)P(R)\\
&= P(Y_{mis}|Y_{obs},R)P(Y_{obs}|R)P(R).\\
\end{align*}
A dataset with missing values contain samples for $Y_{obs}$ and $R$ generated according to some ground truth joint distribution $P_{true}(Y,R)$. An imputation algorithm generates samples from an estimate of $\hat{P}(Y_{mis}|Y_{obs},R)$. Note that the remaining two terms in the joint distribution, $P(Y_{obs}|R)$ and $P(R)$, do not depend on imputation. If we can compare $P_{true}(Y_{mis}|Y_{obs},R)$ to $\hat{P}(Y_{mis}|Y_{obs},R)$ estimated by an imputation algorithm, then it is possible to quantify how good the imputation is. Therefore the imputation evaluation problem can be turned into a problem of comparing two distributions, for which principled quantitative evaluation is possible. From this connection to distribution comparison, we develop a framework for evaluating imputations that can be tractably applied to real-world datasets. 

\noindent\textbf{Problem setup:} We have 1) a dataset with values missing according to some (possibly unknown) missingness model, and 2) the output of $K$ different imputation algorithms, with each one producing multiple filled-in versions of the dataset. The goal is to rank the $K$ algorithms according to a chosen metric. (Several metric choices are discussed in section~\ref{sec:}). 

\noindent\textbf{Assumption:} It should be possible to estimate a model of $P_{true}(Y_{mis}|Y_{obs},R)$ from the data for each unique missingness pattern $R$. Section~\ref{sec:} shows how this can be done tractably. The samples given by an imputation algorithm from its estimated conditional $\hat{P}(Y_{mis}|Y_{obs},R)$ are then compared against this model, rather than the original data itself.

\noindent\textbf{Algorithm:} The main steps are the following:\\
\begin{itemize}
\item A) Construct a model for $P_{true}(Y_{mis}|Y_{obs},R)$ for each unique $R$ in the dataset.
\item B) For each row of the dataset:
\begin{enumerate}
\item Generate samples from the model of $P_{true}(Y_{mis}|Y_{obs},R)$. 
\item Generate samples from the conditional $\hat{P_k}(Y_{mis}|Y_{obs},R)$ estimated by the $k^{th}$ imputation algorithm for the current row.
\item Compute the score $s_k$ for the $k^{th}$ algorithm according to the chosen evaluation metric that compares the two conditional distributions using their corresponding samples.
\item Sort the scores to rank the $K$ algorithms for the current row.
\end{enumerate}
\item C) Use the method recommended by Demsar \cite{dem06} to combine the rankings for all the rows into a single average ranking over the $K$ algorithms. Confidence intervals are assigned to the average ranks to indicate which algorithms are significantly different.
\end{itemize}

There are several choices possible for 1) the model of $P_{true}(Y_{mis}|Y_{obs},R)$, and 2) the metric for distribution comparison. Our evaluation framework is general in that it is not tied to any specific choice for either of these. Nevertheless in section~\ref{sec:} we discuss a few specific choices that are tractable and work well for high-dimensional data. For modeling $P_{true}(Y_{mis}|Y_{obs},R)$ we consider a Conditional Random Field-based approach, as well as propose a novel Markov Random Field-based approach to efficiently learn models for each unique $R$ in a joint manner. For distribution comparison metrics we consider 1) Kullback-Leibler (KL) divergence, 2) Symmetric KL divergence, and 3) two-sample testing for equality of two distributions. Recent advances in kernel-based approaches to estimating these metrics have now made it possible to apply them to high-dimensional data. We estimate KL divergence using the convex risk minimization approach of Nguyen et al. [ref], symmetric KL using the cost-sensitive binary classification approach of Reid and Williamson [ref], and perform two-sample testing using Maximum Mean Discrepancy (MMD) [ref]. In addition, we have proposed a new metric called Neighborhood-based Dissimilarity Score (NDS) that is faster to compute while providing similar results. We demonstrate the framework on several real datasets to compare four representative imputation algorithms from the literature. 

\noindent\textbf{Contributions:} To our knowledge this is the first work that defines
\begin{itemize}
\item A principled framework for computing quantitative metrics to evaluate imputations and rank algorithms with statistical significance tests. Its generality allows different choices for distribution modeling and distribution comparison metrics to be plugged in according to the problem.
\item An efficient algorithm for jointly building distribution models for each unique missingness pattern.
\item Neighborhood-based Dissimilarity Score, which is two orders of magnitude faster than KL, symmetric KL and MMD, while giving similar results.
\end{itemize}
Several things that were previously not possible to do in a principled way now become possible. Using our framework one can now perform evaluation studies that try to characterize which imputation algorithms perform well on what types of datasets, or try to understand the sensitivity of various imputation algorithms to different missingness models. The experiments presented in this paper are a first step towards such deeper investigations.

\noindent\textbf{Notes:} 1) The evaluation does not require knowledge of the missingness model, such as whether values are Missing Completely at Random (MCAR) or Not Missing at Random (NMAR) [ref]. It simply checks whether the samples generated by the imputation algorithm are distributed correctly compared to the true distribution. The imputation algorithm needs to be aware of the missingness model, but not the evaluation. 2) In our experiments we only consider up to 50\% missingness. Imputation is typically used for problems where the missingness percentage is not very high. At much higher percentages, e.g. 99\% missingness in Collaborative Filtering datasets, more specialized approaches are used and evaluation is focused more on predicting a few relevant missing entries rather than \emph{all} of them.

\noindent\textbf{Outline:} Section 2 presents two motivating examples that demonstrate our evaluation framework on datasets where it is possible to visually check the quality of the imputations. Section 3 explains the details of constructing the distribution models, the metrics used for comparing distributions, and statistical significance testing for the ranking of the algorithms. Section 4 presents the experimental results on several datasets, followed by discussion in section 5.

%We make use of recently developed kernel-based techniques for comparing distributions that have been shown to scale well to high-dimensional data.
%We give a high-level overview of the procedure for computing the evaluation metrics.

%In addition to a principled framework for defining quantitative metrics for imputation

%such as estimating divergences between two high-dimensional distributions from samples, and deciding whether two sets of samples came from the same distribution or not. Mention Wainwright-Jordan, Reid-Williamson, Gretton MMD. Kernel based approaches that scale well to high-dimensional data.

%Recent techniques developed in the machine learning literature for 
%What has made our work possible are recent advances in estimating divergences between high-dimensional distributions using only samples from them, as well as tests for deciding whether two distributions are same or not. The 

%The primary contributions of the paper are showing the reduction (defining a framework) and defining a practical procedure for implementing the framework.

%- this approach has become possible due to the recent advances in computing divergences from samples
%- you want to make it sound like this is direct consequence of new exciting developments in ML, and that it was not possible before
%- recent advances in computing divergences between distributions via samples and testing whether samples came from the same distribution

%In practice it need not always be possible to have $P_{true}(Y_{mis}|Y_{obs},R)$. To define a quantitative metric, we need access to the groundtruth distribution that generated the data. Suppose we have a fully-observed dataset on which missingness is introduced synthetically by removing values according to some missingness mechanism. Apply $K$ different imputation algorithms to fill in the missing values, with multiple samples per missing variable to reflect the uncertainty in the imputations. What is the ranking of the $K$ algorithms in terms of the quality of the imputations they produce? This is the problem setup we are considering in this paper.

%The contributions of the paper are:
%\begin{enumerate}
%\item A formalization of what is a ``good imputation'' for the task-independent setting.
%\item We propose a practical procedure for measuring the quality of the imputation.
%\item We propose a new metric YAM for evaluating the imputation quality which is fast and provides consistent rankings.
%\end{enumerate}

%Main points to be made:\\
%1. Missing value imputation is an important problem. There are many algorithms for imputing missing values, but measuring the quality of the imputation is difficult.
%2. If there is a specific task to be solved afterwards, then we can measure quality against that task's evaluation. But if there isn't such a task, how to evaluate is a difficult problem. And such scenarios are becoming more important with generic imputation algorithms.
%3. Hamming distance or Euclidean distance doesn't capture the uncertainty. Rubin supports this. Visually comparing the histograms can be misleading. People have only specified qualitative criteria for evaluation.
%4. We propose quantitative criteria for evaluating the quality of an imputation.
%5. These criteria can only be used with simulated missingness and fully observed data. If you have a model for the missingness mechanism (either MCAR, or NMAR), one can try to measure which algorithm is best suited for that missingness mechanism. Our work now makes it possible to characterize imputation algorithms by the dataset characteristics and missingness mechanisms that they work well on.

%Emphasize that our metrics are agnostic to whatever simplifying assumptions made by the imputation algorithms, like MCAR. The metrics work regardless of such assumptions. This will be a major question in the mind of the reviewers even before reading. Need to make sure they understand that the MCAR/NMAR issue is orthogonal to what we are looking at.

%Missing value imputation is a very important problem in ML. With the increasing use of ML by non-experts, there is a need for black-box solutions for handling missing values. There have been many imputation algorithms proposed in the literature. But there has not been a systematic evaluation of these algorithms. This is partly due to the lack of clear metrics that can be used to evaluate imputation algorithms.

%Distinguish between task-specific imputation versus task-independent imputation.

%- no evaluation of imputation algorithms available due to lack of metrics\\
%- what is a good imputation? Rubin says any downstream analysis should be unable to distinguish the groundtruth distribution from the distribution given by the imputation algorithm\\

%CONTRIBUTIONS:\\
%1. A formalization of what is a "good imputation" for the task-independent setting. This is currently missing in the stats/ML literature. Rubin and Van Buuren gives qualitative criteria for goodness, but no formal definition. (What?) Emphasize the ranking part, we are not claiming that we can say something about the absolute goodness of an imputation algorithm. We are only ranking imputation algorithms. (This issue should be discussed in the paper.)
%2. We apply metrics for computing similarity between distributions via samples to the imputation setting. (How?)
%3. We propose a practical procedure for measuring the quality of the imputation according to the definition in 1. (How?)
%4. We do a empirical comparison of four representative imputation algorithms that have been proposed in the literature. Don't overstate this --we haven't done an exhaustive evaluation. Mention how we validate the evaluation.
%5. We propose a new metric YAM for evaluating the imputation quality which is fast and provides consistent rankings.

